Yukawa Unification in an SO(10) SUSY GUT: SUSY on the Edge

In this paper we analyze Yukawa unification in a three family SO(10) SUSY GUT. We perform a global $\chi^2$ analysis and show that SUSY effects do not decouple even though the universal scalar mass parameter at the GUT scale, $m_{16}$, is found to lie between 15 and 30 TeV with the best fit given for $m_{16} \approx 25$ TeV. Note, SUSY effects don't decouple since stops and bottoms have mass of order 5 TeV, due to RG running from $M_{GUT}$. The model has many testable predictions. Gauginos are the lightest sparticles and the light Higgs boson is very much Standard Model-like. The model is consistent with flavor and CP observables with the $BR(\mu \to e\gamma)$ close to the experimental upper bound. With such a large value of $m_{16}$ we clearly cannot be considered "natural" SUSY nor are we "Split" SUSY. We are thus in the region in between or "SUSY on the Edge."

==> SO(10) New/tables/benchmark.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 25 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!htbp]\footnotesize
  \caption{Benchmark point with $m_{16} = 25\ \text{TeV}, M_{\tilde g} = 1.202\ \text{TeV}, \alpha=0$:}
  \label{tab:fit25}
  $(1/\alpha_G, M_G, \epsilon_3) = (25.98, 2.55\times10^{16}\ \text{GeV}, -1.30\%)$\\
  $(\lambda, \lambda\epsilon, \sigma, \lambda\tilde\epsilon, \rho, \lambda\epsilon', \lambda\epsilon\xi) = (0.6101, 0.0308, 1.1559, 0.0049, 0.0698, -0.0019, 0.0036)$\\
  $(\phi_\sigma, \phi_{\tilde\epsilon}, \phi_{\rho}, \phi_\xi) = (0.52, 0.58, 3.95, 3.47)\text{rad}$\\
  $(m_{16}, M_{1/2}, A_0, \mu(M_Z)) = (25000, 280, -51380, 1212)\ \text{GeV}$\\
  $((m_{H_d}/m_{16})^2, (m_{H_u}/m_{16})^2, \tan\beta) = (1.86, 1.61, 50.29)$\\
  $(M_{R_1}, M_{R_2}, M_{R_3}) = (9.2, 578.8, 35054.2)\ \times10^9\text{GeV}$

  \begin{center}
    \scalebox{0.8}{
      \begin{tabular}{|l|r|r|r|r|}
        \hline
        Observable & Fit & Exp. & Pull & $\sigma$ \\
        \hline\hline
        $M_Z$ & 91.1876 & 91.1876 & 0.0000 & 0.4541 \\
        $M_W$ & 80.4784 & 80.3850 & 0.2320 & 0.4027 \\
        $1/\alpha_\text{em}$ &  137.2810 & 0.0073 & 0.3569 & 0.6864 \\
        $G_\mu\times10^5$ & 1.1789 & 1.1664 & 1.0598 & 0.0118 \\
        $\alpha_3(M_Z)$ & 0.1192 & 0.1185 & 0.8199 & 0.0008 \\
        \hline
        $M_t$ & 174.0947 & 173.2100 & 0.7171 & 1.2337 \\
        $m_b(m_b)$ & 4.1986 & 4.1800 & 0.5092 & 0.0366 \\
        $m_\tau$ & 1.7772 & 1.7768 & 0.0428 & 0.0089 \\
        \hline
        $M_b-M_c$ & 3.1701 & 3.4500 & 0.8720 & 0.3209 \\
        $m_c(m_c)$ & 1.2509 & 1.2750 & 0.9333 & 0.0258 \\
        $m_s(2\ \text{GeV})$ & 0.0953 & 0.0950 & 0.0609 & 0.0050 \\
        $m_d/m_s(2\ \text{GeV})$  & 0.0702 & 0.0513 & 2.8247 & 0.0067 \\
        $1/Q^2$ & 0.0018 & 0.0019 & 0.4528 & 0.0001 \\
        $M_\mu$ & 0.1056 & 0.1057 & 0.0578 & 0.0005 \\
        $M_e\times10^4$ & 5.1143 & 5.1100 & 0.1674 & 0.0256 \\
        \hline
        $|V_{us}|$ & 0.2245 & 0.2253 & 0.5931 & 0.0014 \\
        $|V_{cb}|$ & 0.0404 & 0.0408 & 0.1670 & 0.0021 \\
        $|V_{ub}|\times10^3$ & 3.1235 & 3.8500 & 0.8446 & 0.8601 \\
        $|V_{td}|\times10^3$ & 8.8463 & 8.4000 & 0.7418 & 0.6016 \\
        $|V_{ts}|$ & 0.0396 & 0.0400 & 0.1508 & 0.0027 \\
        $\sin2\beta$ & 0.6296 & 0.6820 & 2.7214 & 0.0193 \\
        $\epsilon_K$ & 0.0022 & 0.0022 & 0.0022 & 0.0002 \\
        \hline
        $\Delta M_{B_s}/\Delta M_{B_d}$ & 34.8195 & 35.0345 & 0.0308 & 6.9747 \\
        $\Delta M_{B_d}\times10^{13}$ & 3.9946 & 3.3370 & 0.8224 & 0.7996 \\
        \hline
        $m^2_{21}\times10^5$ &   7.5883 & 7.5550 & 0.0621 & 0.5363 \\
        $m^2_{31}\times10^3$ &  2.4649 & 2.4620 & 0.0197 & 0.1455 \\
        $\sin^2\theta_{12}$ & 0.3028 & 0.3070 & 0.1125 & 0.0370 \\
        $\sin^2\theta_{23}$ & 0.6600 & 0.5125 & 1.1300 & 0.1305 \\
        $\sin^2\theta_{13}$ & 0.0162 & 0.0218 & 1.7510 & 0.0032 \\
        \hline
        $M_h$ & 126.2697 & 125.7000 & 0.1882 & 3.0265 \\
        \hline
        $BR(B\to s\gamma)\times10^4$ & 2.7220 & 3.4300 & 0.5419 & 1.3064 \\
        $BR(B_s\to\mu^+\mu^-)\times10^9$ & 2.7213 & 2.8000 & 0.0888 & 0.8867 \\
        $BR(B_d\to\mu^+\mu^-)\times10^{10}$ & 1.0734 & 3.9000 & 1.7509 & 1.6143 \\
        $BR(B\to\tau\nu)\times10^5$ & 6.2223 & 11.4000 & 1.3588 & 3.8104 \\
        \hline
        $BR(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}\times10^8$ & 4.7860 & 3.4000 & 0.2739 & 5.0610 \\
        $BR(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq 16\ \text{GeV}^2}\times10^8$ & 7.5495 & 5.6000 & 0.1356 & 14.3788 \\
        $q_0^2(A_\text{FB}(B\to K^*\mu^+\mu^-))$ & 3.7120 & 4.9000 & 0.9190 & 1.2927 \\
        $F_L(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.7207 & 0.6500 & 0.2101 & 0.3366 \\
        $F_L(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & 0.3108 & 0.3300 & 0.0726 & 0.2644 \\
        $P_2(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.0331 & 0.3300 & 2.3939 & 0.1240 \\
        $P_2(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & -0.4336 & -0.5000 & 0.3364 & 0.1974 \\
        $P_4'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.5717 & 0.5800 & 0.0208 & 0.3988 \\
        $P_4'(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & 1.2190 & -0.1800 & 1.7066 & 0.8198 \\
        $P_5'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & -0.4335 & 0.2100 & 2.2451 & 0.2866 \\
        $P_5'(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & -0.7116 & -0.7900 & 0.1552 & 0.5052 \\
        \hline
        \multicolumn{3}{|l|}{Total $\chi^2$} & 46.7692 & \\
        \hline
      \end{tabular}
    }
  \end{center}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 25A %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!htbp]\small
  \caption{Benchmark point with $m_{16} = 25\ \text{TeV}, M_{\tilde g} = 1.187\ \text{TeV}, \alpha=1.5$:}
  \label{tab:fit25A}
  $(1/\alpha_G, M_G, \epsilon_3) = (25.95, 2.60\times10^{16}\ \text{GeV}, -1.50\%)$\\
  $(\lambda, \lambda\epsilon, \sigma, \lambda\tilde\epsilon, \rho, \lambda\epsilon', \lambda\epsilon\xi) = (0.6100, 0.0310, 1.1459, 0.0049, 0.0708, -0.0019, 0.0037)$\\
  $(\phi_\sigma, \phi_{\tilde\epsilon}, \phi_{\rho}, \phi_\xi) = (0.53, 0.57, 3.94, 3.49)\text{rad}$\\
  $(m_{16}, M_{1/2}, A_0, \mu(M_Z)) = (25000, 520, -51157, 1236)\ \text{GeV}$\\
  $((m_{H_d}/m_{16})^2, (m_{H_u}/m_{16})^2, \tan\beta) = (1.85, 1.61, 50.19)$\\
  $(M_{R_1}, M_{R_2}, M_{R_3}) = (9.1, 567.0, 32370.5)\ \times10^9\text{GeV}$

  \begin{center}
    \scalebox{0.8}{
      \begin{tabular}{|l|r|r|r|r|}
        \hline
        Observable & Fit & Exp. & Pull & $\sigma$ \\
        \hline\hline
        $M_Z$ & 91.1876 & 91.1876 & 0.0000 & 0.4540 \\
        $M_W$ & 80.5197 & 80.3850 & 0.3344 & 0.4029 \\
        $1/\alpha_\text{em}$ &  137.1416 & 0.0073 & 0.1540 & 0.6857 \\
        $G_\mu\times10^5$ & 1.1829 & 1.1664 & 1.3978 & 0.0118 \\
        $\alpha_3(M_Z)$ & 0.1189 & 0.1185 & 0.4798 & 0.0008 \\
        \hline
        $M_t$ & 173.8449 & 173.2100 & 0.5150 & 1.2328 \\
        $m_b(m_b)$ & 4.2023 & 4.1800 & 0.6094 & 0.0366 \\
        $m_\tau$ & 1.7772 & 1.7768 & 0.0450 & 0.0089 \\
        \hline
        $M_b-M_c$ & 3.1680 & 3.4500 & 0.8791 & 0.3207 \\
        $m_c(m_c)$ & 1.2570 & 1.2750 & 0.6979 & 0.0258 \\
        $m_s(2\ \text{GeV})$ & 0.0947 & 0.0950 & 0.0671 & 0.0050 \\
        $m_d/m_s(2\ \text{GeV})$  & 0.0700 & 0.0513 & 2.7901 & 0.0067 \\
        $1/Q^2$ & 0.0018 & 0.0019 & 0.5027 & 0.0001 \\
        $M_\mu$ & 0.1056 & 0.1057 & 0.1457 & 0.0005 \\
        $M_e\times10^4$ & 5.1145 & 5.1100 & 0.1775 & 0.0256 \\
        \hline
        $|V_{us}|$ & 0.2244 & 0.2253 & 0.6440 & 0.0014 \\
        $|V_{cb}|$ & 0.0407 & 0.0408 & 0.0584 & 0.0021 \\
        $|V_{ub}|\times10^3$ & 3.1307 & 3.8500 & 0.8363 & 0.8601 \\
        $|V_{td}|\times10^3$ & 8.8596 & 8.4000 & 0.7639 & 0.6016 \\
        $|V_{ts}|$ & 0.0398 & 0.0400 & 0.0652 & 0.0027 \\
        $\sin2\beta$ & 0.6285 & 0.6820 & 2.7790 & 0.0193 \\
        $\epsilon_K$ & 0.0023 & 0.0022 & 0.1149 & 0.0002 \\
        \hline
        $\Delta M_{B_s}/\Delta M_{B_d}$ & 35.5946 & 35.0345 & 0.0786 & 7.1295 \\
        $\Delta M_{B_d}\times10^{13}$ & 3.9756 & 3.3370 & 0.8025 & 0.7958 \\
        \hline
        $m^2_{21}\times10^5$ &   7.6111 & 7.5550 & 0.1046 & 0.5364 \\
        $m^2_{31}\times10^3$ &  2.4657 & 2.4620 & 0.0255 & 0.1455 \\
        $\sin^2\theta_{12}$ & 0.3134 & 0.3070 & 0.1724 & 0.0370 \\
        $\sin^2\theta_{23}$ & 0.6319 & 0.5125 & 0.9146 & 0.1305 \\
        $\sin^2\theta_{13}$ & 0.0153 & 0.0218 & 2.0337 & 0.0032 \\
        \hline
        $M_h$ & 124.5455 & 125.7000 & 0.3814 & 3.0265 \\
        \hline
        $BR(B\to s\gamma)\times10^4$ & 2.7270 & 3.4300 & 0.5372 & 1.3087 \\
        $BR(B_s\to\mu^+\mu^-)\times10^9$ & 2.5215 & 2.8000 & 0.3228 & 0.8627 \\
        $BR(B_d\to\mu^+\mu^-)\times10^{10}$ & 1.0192 & 3.9000 & 1.7861 & 1.6129 \\
        $BR(B\to\tau\nu)\times10^5$ & 6.2272 & 11.4000 & 1.3568 & 3.8124 \\
        \hline
        $BR(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}\times10^8$ & 4.8580 & 3.4000 & 0.2839 & 5.1361 \\
        $BR(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq 16\ \text{GeV}^2}\times10^8$ & 7.6648 & 5.6000 & 0.1415 & 14.5975 \\
        $q_0^2(A_\text{FB}(B\to K^*\mu^+\mu^-))$ & 3.7150 & 4.9000 & 0.9163 & 1.2933 \\
        $F_L(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.7208 & 0.6500 & 0.2103 & 0.3366 \\
        $F_L(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & 0.3108 & 0.3300 & 0.0726 & 0.2644 \\
        $P_2(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.0335 & 0.3300 & 2.3879 & 0.1242 \\
        $P_2(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & -0.4336 & -0.5000 & 0.3364 & 0.1974 \\
        $P_4'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.5697 & 0.5800 & 0.0258 & 0.3985 \\
        $P_4'(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & 1.2190 & -0.1800 & 1.7066 & 0.8198 \\
        $P_5'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & -0.4334 & 0.2100 & 2.2450 & 0.2866 \\
        $P_5'(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & -0.7117 & -0.7900 & 0.1550 & 0.5052 \\
        \hline
        \multicolumn{3}{|l|}{Total $\chi^2$} & 47.7692 & \\
        \hline
      \end{tabular}
    }
  \end{center}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 25 1.6 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!htbp]\small
  \caption{Benchmark point with $m_{16} = 25\ \text{TeV}, M_{\tilde g} = 1.613\ \text{TeV}, \alpha=0$:}
  \label{tab:fit25A}
  $(1/\alpha_G, M_G, \epsilon_3) = (26.22, 2.32\times10^{16}\ \text{GeV}, -0.65\%)$\\
  $(\lambda, \lambda\epsilon, \sigma, \lambda\tilde\epsilon, \rho, \lambda\epsilon', \lambda\epsilon\xi) = (0.6096, 0.0311, 1.1398, 0.0049, 0.0710, -0.0019, 0.0038)$\\
  $(\phi_\sigma, \phi_{\tilde\epsilon}, \phi_{\rho}, \phi_\xi) = (0.53, 0.56, 3.95, 3.49)\text{rad}$\\
  $(m_{16}, M_{1/2}, A_0, \mu(M_Z)) = (25000, 450, -51341, 1226)\ \text{GeV}$\\
  $((m_{H_d}/m_{16})^2, (m_{H_u}/m_{16})^2, \tan\beta) = (1.86, 1.61, 50.30)$\\
  $(M_{R_1}, M_{R_2}, M_{R_3}) = (9.1, 572.4, 32277.4)\ \times10^9\text{GeV}$

  \begin{center}
    \scalebox{0.8}{
      \begin{tabular}{|l|r|r|r|r|}
        \hline
        Observable & Fit & Exp. & Pull & $\sigma$ \\
        \hline\hline
        $M_Z$ & 91.1876 & 91.1876 & 0.0000 & 0.4535 \\
        $M_W$ & 80.4507 & 80.3850 & 0.1633 & 0.4025 \\
        $1/\alpha_\text{em}$ &  137.7125 & 0.0073 & 0.9825 & 0.6886 \\
        $G_\mu\times10^5$ & 1.1732 & 1.1664 & 0.5798 & 0.0117 \\
        $\alpha_3(M_Z)$ & 0.1188 & 0.1185 & 0.4140 & 0.0008 \\
        \hline
        $M_t$ & 174.1882 & 173.2100 & 0.7927 & 1.2340 \\
        $m_b(m_b)$ & 4.1954 & 4.1800 & 0.4220 & 0.0366 \\
        $m_\tau$ & 1.7781 & 1.7768 & 0.1417 & 0.0089 \\
        \hline
        $M_b-M_c$ & 3.1568 & 3.4500 & 0.9175 & 0.3196 \\
        $m_c(m_c)$ & 1.2595 & 1.2750 & 0.5993 & 0.0258 \\
        $m_s(2\ \text{GeV})$ & 0.0939 & 0.0950 & 0.2147 & 0.0050 \\
        $m_d/m_s(2\ \text{GeV})$  & 0.0701 & 0.0513 & 2.8052 & 0.0067 \\
        $1/Q^2$ & 0.0018 & 0.0019 & 0.5139 & 0.0001 \\
        $M_\mu$ & 0.1056 & 0.1057 & 0.1818 & 0.0005 \\
        $M_e\times10^4$ & 5.1145 & 5.1100 & 0.1749 & 0.0256 \\
        \hline
        $|V_{us}|$ & 0.2244 & 0.2253 & 0.6763 & 0.0014 \\
        $|V_{cb}|$ & 0.0404 & 0.0408 & 0.1729 & 0.0021 \\
        $|V_{ub}|\times10^3$ & 3.1033 & 3.8500 & 0.8681 & 0.8601 \\
        $|V_{td}|\times10^3$ & 8.8101 & 8.4000 & 0.6817 & 0.6016 \\
        $|V_{ts}|$ & 0.0396 & 0.0400 & 0.1531 & 0.0027 \\
        $\sin2\beta$ & 0.6270 & 0.6820 & 2.8562 & 0.0193 \\
        $\epsilon_K$ & 0.0022 & 0.0022 & 0.2052 & 0.0002 \\
        \hline
        $\Delta M_{B_s}/\Delta M_{B_d}$ & 35.3739 & 35.0345 & 0.0479 & 7.0854 \\
        $\Delta M_{B_d}\times10^{13}$ & 3.9433 & 3.3370 & 0.7681 & 0.7894 \\
        \hline
        $m^2_{21}\times10^5$ &   7.6562 & 7.5550 & 0.1886 & 0.5364 \\
        $m^2_{31}\times10^3$ &  2.4631 & 2.4620 & 0.0077 & 0.1455 \\
        $\sin^2\theta_{12}$ & 0.3170 & 0.3070 & 0.2689 & 0.0370 \\
        $\sin^2\theta_{23}$ & 0.6264 & 0.5125 & 0.8722 & 0.1305 \\
        $\sin^2\theta_{13}$ & 0.0149 & 0.0218 & 2.1658 & 0.0032 \\
        \hline
        $M_h$ & 124.5054 & 125.7000 & 0.3947 & 3.0265 \\
        \hline
        $BR(B\to s\gamma)\times10^4$ & 2.6840 & 3.4300 & 0.5789 & 1.2887 \\
        $BR(B_s\to\mu^+\mu^-)\times10^9$ & 3.0247 & 2.8000 & 0.2429 & 0.9252 \\
        $BR(B_d\to\mu^+\mu^-)\times10^{10}$ & 1.1022 & 3.9000 & 1.7323 & 1.6151 \\
        $BR(B\to\tau\nu)\times10^5$ & 6.1884 & 11.4000 & 1.3727 & 3.7966 \\
        \hline
        $BR(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}\times10^8$ & 4.7640 & 3.4000 & 0.2707 & 5.0381 \\
        $BR(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq 16\ \text{GeV}^2}\times10^8$ & 7.5110 & 5.6000 & 0.1336 & 14.3059 \\
        $q_0^2(A_\text{FB}(B\to K^*\mu^+\mu^-))$ & 3.6690 & 4.9000 & 0.9579 & 1.2850 \\
        $F_L(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.7225 & 0.6500 & 0.2149 & 0.3374 \\
        $F_L(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & 0.3108 & 0.3300 & 0.0726 & 0.2644 \\
        $P_2(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.0228 & 0.3300 & 2.5196 & 0.1219 \\
        $P_2(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & -0.4336 & -0.5000 & 0.3364 & 0.1974 \\
        $P_4'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.5820 & 0.5800 & 0.0050 & 0.4001 \\
        $P_4'(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & 1.2190 & -0.1800 & 1.7066 & 0.8198 \\
        $P_5'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & -0.4455 & 0.2100 & 2.2578 & 0.2903 \\
        $P_5'(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & -0.7116 & -0.7900 & 0.1552 & 0.5052 \\
        \hline
        \multicolumn{3}{|l|}{Total $\chi^2$} & 48.8413 & \\
        \hline
      \end{tabular}
    }
  \end{center}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 25A 1.6 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!htbp]\small
  \caption{Benchmark point with $m_{16} = 25\ \text{TeV}, M_{\tilde g} = 1.690\ \text{TeV}, \alpha=1.5$:}
  \label{tab:fit25A}
  $(1/\alpha_G, M_G, \epsilon_3) = (26.38, 2.09\times10^{16}\ \text{GeV}, 0.02\%)$\\
  $(\lambda, \lambda\epsilon, \sigma, \lambda\tilde\epsilon, \rho, \lambda\epsilon', \lambda\epsilon\xi) = (0.6096, 0.0311, 1.1384, 0.0049, 0.0708, -0.0019, 0.0037)$\\
  $(\phi_\sigma, \phi_{\tilde\epsilon}, \phi_{\rho}, \phi_\xi) = (0.52, 0.56, 3.96, 3.49)\text{rad}$\\
  $(m_{16}, M_{1/2}, A_0, \mu(M_Z)) = (25000, 900, -50846, 1529)\ \text{GeV}$\\
  $((m_{H_d}/m_{16})^2, (m_{H_u}/m_{16})^2, \tan\beta) = (1.86, 1.60, 50.31)$\\
  $(M_{R_1}, M_{R_2}, M_{R_3}) = (9.1, 579.0, 32367.3)\ \times10^9\text{GeV}$

  \begin{center}
    \scalebox{0.8}{
      \begin{tabular}{|l|r|r|r|r|}
        \hline
        Observable & Fit & Exp. & Pull & $\sigma$ \\
        \hline\hline
        $M_Z$ & 91.1876 & 91.1876 & 0.0000 & 0.4540 \\
        $M_W$ & 80.4655 & 80.3850 & 0.2000 & 0.4026 \\
        $1/\alpha_\text{em}$ &  137.7323 & 0.0073 & 1.0111 & 0.6887 \\
        $G_\mu\times10^5$ & 1.1740 & 1.1664 & 0.6469 & 0.0117 \\
        $\alpha_3(M_Z)$ & 0.1188 & 0.1185 & 0.2979 & 0.0008 \\
        \hline
        $M_t$ & 174.3427 & 173.2100 & 0.9175 & 1.2345 \\
        $m_b(m_b)$ & 4.2001 & 4.1800 & 0.5479 & 0.0366 \\
        $m_\tau$ & 1.7774 & 1.7768 & 0.0644 & 0.0089 \\
        \hline
        $M_b-M_c$ & 3.1659 & 3.4500 & 0.8863 & 0.3205 \\
        $m_c(m_c)$ & 1.2574 & 1.2750 & 0.6825 & 0.0258 \\
        $m_s(2\ \text{GeV})$ & 0.0936 & 0.0950 & 0.2741 & 0.0050 \\
        $m_d/m_s(2\ \text{GeV})$  & 0.0701 & 0.0513 & 2.8082 & 0.0067 \\
        $1/Q^2$ & 0.0018 & 0.0019 & 0.5170 & 0.0001 \\
        $M_\mu$ & 0.1056 & 0.1057 & 0.1571 & 0.0005 \\
        $M_e\times10^4$ & 5.1139 & 5.1100 & 0.1545 & 0.0256 \\
        \hline
        $|V_{us}|$ & 0.2244 & 0.2253 & 0.6688 & 0.0014 \\
        $|V_{cb}|$ & 0.0400 & 0.0408 & 0.3609 & 0.0021 \\
        $|V_{ub}|\times10^3$ & 3.0662 & 3.8500 & 0.9113 & 0.8601 \\
        $|V_{td}|\times10^3$ & 8.7156 & 8.4000 & 0.5247 & 0.6016 \\
        $|V_{ts}|$ & 0.0392 & 0.0400 & 0.2960 & 0.0027 \\
        $\sin2\beta$ & 0.6259 & 0.6820 & 2.9122 & 0.0193 \\
        $\epsilon_K$ & 0.0022 & 0.0022 & 0.0834 & 0.0002 \\
        \hline
        $\Delta M_{B_s}/\Delta M_{B_d}$ & 34.7964 & 35.0345 & 0.0342 & 6.9701 \\
        $\Delta M_{B_d}\times10^{13}$ & 3.8958 & 3.3370 & 0.7165 & 0.7799 \\
        \hline
        $m^2_{21}\times10^5$ &   7.6614 & 7.5550 & 0.1984 & 0.5364 \\
        $m^2_{31}\times10^3$ &  2.4606 & 2.4620 & 0.0094 & 0.1455 \\
        $\sin^2\theta_{12}$ & 0.3197 & 0.3070 & 0.3423 & 0.0370 \\
        $\sin^2\theta_{23}$ & 0.6197 & 0.5125 & 0.8210 & 0.1305 \\
        $\sin^2\theta_{13}$ & 0.0146 & 0.0218 & 2.2520 & 0.0032 \\
        \hline
        $M_h$ & 122.0502 & 125.7000 & 1.2059 & 3.0265 \\
        \hline
        $BR(B\to s\gamma)\times10^4$ & 2.6310 & 3.4300 & 0.6321 & 1.2640 \\
        $BR(B_s\to\mu^+\mu^-)\times10^9$ & 3.5145 & 2.8000 & 0.7203 & 0.9920 \\
        $BR(B_d\to\mu^+\mu^-)\times10^{10}$ & 1.0522 & 3.9000 & 1.7647 & 1.6138 \\
        $BR(B\to\tau\nu)\times10^5$ & 6.1009 & 11.4000 & 1.4090 & 3.7610 \\
        \hline
        $BR(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}\times10^8$ & 4.6780 & 3.4000 & 0.2583 & 4.9484 \\
        $BR(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq 16\ \text{GeV}^2}\times10^8$ & 7.4066 & 5.6000 & 0.1281 & 14.1080 \\
        $q_0^2(A_\text{FB}(B\to K^*\mu^+\mu^-))$ & 3.6290 & 4.9000 & 0.9946 & 1.2779 \\
        $F_L(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.7240 & 0.6500 & 0.2189 & 0.3380 \\
        $F_L(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & 0.3108 & 0.3300 & 0.0726 & 0.2644 \\
        $P_2(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.0132 & 0.3300 & 2.6254 & 0.1207 \\
        $P_2(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & -0.4337 & -0.5000 & 0.3358 & 0.1975 \\
        $P_4'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.5918 & 0.5800 & 0.0294 & 0.4014 \\
        $P_4'(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & 1.2190 & -0.1800 & 1.7066 & 0.8198 \\
        $P_5'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & -0.4562 & 0.2100 & 2.2685 & 0.2937 \\
        $P_5'(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & -0.7117 & -0.7900 & 0.1550 & 0.5052 \\
        \hline
        \multicolumn{3}{|l|}{Total $\chi^2$} & 52.6056 & \\
        \hline
      \end{tabular}
    }
  \end{center}
\end{table}

==> SO(10) New/tables/fine_tuning_table.tex <==
\begin{table}[!htbp]
  \begin{center}
    \begin{tabular}{| l | r | r | r | r | r |}
      \multicolumn{6}{c}{Fine-Tuning of Benchmark Points with $\alpha=0$ and $M_{\tilde{g}}\approx1.2\ \text{TeV}$}
      \\ \hline
        & \multicolumn{5}{c|}{$m_{16}$}
      \\ \cline{2-6} Varying Parameters & 10TeV & 15TeV & 20TeV & 25TeV & 30TeV
      \\ \hline $\mu$ & 140 & 190 & 210 & 360 & 490
      \\ \hline $M_{1/2}$ & 260 & 340 & 400 & 430 & 450
      \\ \hline $m_{16}$ & 12000 & 27000 & 47000 & 74000 & 110000
      \\ \hline $m_{H_d}$ & 760 & 1500 & 3900 & 6100 & 8700
      \\ \hline $m_{H_u}$ & 10000 & 23000 & 40000 & 62000 & 89000
      \\ \hline $A_0$ & 9300 & 21000 & 39000 & 61000 & 85000
      \\ \hline\hline $m_{16}$ with $A_0/m_{16}$ fixed & 22000 & 49000 & 87000 & 130000 & 190000
      \\ \hline $m_{16}$ with $m_{H_u,d}/m_{16}$ fixed & 9500 & 22000 & 40000 & 62000 & 86000
      \\ \hline\hline $m_{16}$ with $m_{H_{u,d}}/m_{16}, A_0/m_{16}$ fixed & 240 & 400 & 630 & 740 & 850
      \\ \hline \multicolumn{6}{c}{}
      \\ \multicolumn{6}{c}{Fine-Tuning of Benchmark Points with $\alpha=1.5$ and $M_{\tilde{g}}\approx1.2\ \text{TeV}$}
      \\ \hline
        & \multicolumn{5}{c|}{$m_{16}$}
      \\ \cline{2-6} Varying Parameters & 10TeV & 15TeV & 20TeV & 25TeV & 30TeV
      \\ \hline $\mu$ & 110 & 240 & 290 & 340 & 380
      \\ \hline $M_{1/2}$ & 320 & 420 & 500 & 560 & 580
      \\ \hline $m_{16}$ & 12000 & 28000 & 48000 & 74000 & 110000
      \\ \hline $m_{H_d}$ & 750 & 1500 & 4600 & 6000 & 8500
      \\ \hline $m_{H_u}$ & 10000 & 23000 & 39000 & 62000 & 89000
      \\ \hline $A_0$ & 9200 & 21000 & 39000 & 60000 & 86000
      \\ \hline\hline $m_{16}$ with $A_0/m_{16}$ fixed & 22000 & 49000 & 87000 & 130000 & 190000
      \\ \hline $m_{16}$ with $m_{H_u,d}/m_{16}$ fixed & 9600 & 21000 & 39000 & 61000 & 87000
      \\ \hline\hline $m_{16}$ with $m_{H_{u,d}}/m_{16}, A_0/m_{16}$ fixed & 330 & 450 & 670 & 890 & 1100
      \\ \hline
    \end{tabular}
    \caption{Without fixing any ratios, the fine-tuning is 1 part in $10^5$. When the ratio of $m_{H_{u,d}}/m_{16}$ and $A_0/m_{16}$ are fixed, the fine-tuning according to (\ref{eq:ft_bg}) is about 1 part in $500$.  This suggests that these ratios should be fixed in a more fundamental natural theory.  In addition, fine-tuning increases as $m_{16}$ increases.  Hence, in our model, small $m_{16}$ is favored by naturalness.}
    \label{tab:ft}
  \end{center}
\end{table}

==> SO(10) New/tables/input_tab.tex <==
\begin{table}
  \begin{center}
    \renewcommand{\arraystretch}{1.2}
      \scalebox{0.83}{
        \begin{tabular}{|l||c|c||c|c||}
          \hline Sector & Universal Gaugino Masses & No. & Mirage Mediated Gaugino Masses & No.
          \\ \hline Gauge & $\alpha_G$, $M_G$, $\epsilon_3$ & 3 & $\alpha_G$, $M_G$, $\epsilon_3$ & 3
          \\ SUSY (GUT scale) & $m_{16}$, $M_{1/2}$, $A_0$, $m_{H_u}$, $m_{H_d}$
            & 5 & $m_{16}$, $M_{1/2}$, $A_0$, $m_{H_u}$, $m_{H_d}$, $\alpha$ & 6
          \\ Yukawa Textures & $\epsilon$, $\epsilon'$, $\lambda$, $\rho$, $\sigma$, $\tilde\epsilon$, $\xi$, $\phi_{\rho}$, $\phi_{\sigma}$, $\phi_{\tilde\epsilon}$, $\phi_{\xi}$ & 11 & $\epsilon$, $\epsilon'$, $\lambda$, $\rho$, $\sigma$, $\tilde\epsilon$, $\xi$, $\phi_{\rho}$, $\phi_{\sigma}$, $\phi_{\tilde\epsilon}$, $\phi_{\xi}$ & 11
          \\ Neutrino & $M_{R_1}$, $M_{R_2}$, $M_{R_3}$ & 3 & $M_{R_1}$, $M_{R_2}$, $M_{R_3}$ & 3
          \\ SUSY (EW Scale) & $\tan\beta$, $\mu$ & 2 & $\tan\beta$, $\mu$ & 2
          \\ \hline Total & & 24 & & 25
          \\ \hline
        \end{tabular}
      }
    \caption{Our model has 24 free parameters for universal gaugino masses boundary conditions. For mirage mediated gaugino masses boundary condition, there is an additional input parameter, $\alpha$, which determines the amount of splitting of the gaugino masses at GUT scale.}
    \label{tab:inputs}
  \end{center}
\end{table}

==> SO(10) New/tables/obs_table.tex <==
\begin{table}[!htbp]\footnotesize
\begin{center}
\scalebox{0.7}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|l|l|l|l|c|}
\hline
\textbf{Observable} &  \textbf{Exp.~Value}   & \textbf{Ref.}          & \textbf{Program} &  \textbf{Th.~Error}  \\
\hline
\hline
$M_Z$ & $91.1876\pm0.0021\ \text{GeV}$ & \cite{Agashe:2014kda} & Input & $0.0\%$ \\
$M_W$ & $80.385\pm0.015\ \text{GeV}$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$\alpha_\text{em}$ & $1/137.035999074(44)$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$G_\mu$ & $1.1663787(6)\times10^{-5}\ \text{GeV}^{-2}$ & \cite{Agashe:2014kda} & \texttt{maton} & $1\%$ \\
$\alpha_3(M_Z)$ & $0.1185\pm0.0006$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
\hline
$M_t$ & $173.21\pm0.51\pm0.71\ \text{GeV}$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$m_b(m_b)$ & $4.18\pm0.03\ \text{GeV}$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$M_\tau$ & $1776.82\pm0.16\text{ MeV}$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
\hline
$m_b-m_c$ & $3.45\pm0.05\ \text{GeV}$ & \cite{Agashe:2014kda} & \texttt{maton} & $10\%$ \\
$m_c(m_c)$ & $1.275\pm0.025\ \text{GeV}$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$m_s(2\ \text{GeV})$ & $95\pm5\text{ MeV}$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$m_s/m_d\,(2\ \text{GeV})$ & $17-22$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$Q$ & $21-25$ & \cite{Agashe:2014kda} & \texttt{maton} & $5\%$ \\
$M_\mu$ & $105.6583715(35)\text{ MeV}$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$M_e$ & $0.510998928(11)\text{ MeV}$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
\hline
$|V_{us}|$ & $0.2253\pm0.0008$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$|V_{cb}|$ (Inclusive) & $0.0422\pm0.0007$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$|V_{cb}|$ (Exclusive) & $0.0395\pm0.0008$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$|V_{cb}|$ (Both) & $0.0408\pm0.0021$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$|V_{ub}|$ (Inclusive) & $0.00441\pm0.00024$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$|V_{ub}|$ (Exclusive) & $0.00328\pm0.00029$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$|V_{ub}|$ (Both) & $0.00385\pm0.00086$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$|V_{td}|$ & $0.00840\pm0.0006$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$|V_{ts}|$ & $0.0400\pm0.0027$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$\sin2\beta$ & $0.682\pm0.019$ & \cite{Agashe:2014kda} & \texttt{maton} & $0.5\%$ \\
$\epsilon_K$ & $(2.2325\pm0.0155)\times 10^{-3}$ & \cite{Agashe:2014kda} & \texttt{susyflavor}\cite{Crivellin:2012jv} & $10\%$ \\
\hline
$\Delta m_{B_s}/\Delta m_{B_d}$ & $35.0345\pm0.3884$ & \cite{Agashe:2014kda} & \texttt{susyflavor}\cite{Crivellin:2012jv} & $20\%$ \\
$\Delta m_{B_d}$ & $(3.337\pm0.033)\times 10^{-10}\text{ MeV}$ & \cite{Agashe:2014kda} & \texttt{susyflavor}\cite{Crivellin:2012jv} & $20\%$ \\
\hline
$\Delta m_{21}^2$ & $(7.02-8.09)\times10^{-5}\text{ eV}^2$ (3$\sigma$ range) & \cite{Gonzalez-Garcia:2014bfa} & \texttt{maton} & $0.5\%$ \\
$\Delta m_{31}^2$ & $(2.317-2.607)\times10^{-3}\text{ eV}^2$ (3$\sigma$ range) & \cite{Gonzalez-Garcia:2014bfa} & \texttt{maton} & $0.5\%$ \\
$\sin^2\theta_{12}$ & $0.270-0.344$ (3$\sigma$ range) & \cite{Gonzalez-Garcia:2014bfa} & \texttt{maton} & $0.5\%$ \\
$\sin^2\theta_{23}$ & $0.382-0.643$ (3$\sigma$ range) & \cite{Gonzalez-Garcia:2014bfa} & \texttt{maton} & $0.5\%$ \\
$\sin^2\theta_{13}$ & $0.0186-0.0250$ (3$\sigma$ range) & \cite{Gonzalez-Garcia:2014bfa} & \texttt{maton} & $0.5\%$ \\
\hline
$M_h$ & $125.7\pm0.4\ \text{GeV}$ & \cite{Agashe:2014kda} & \texttt{splitsuspect}\cite{Bernal:2007uv} & $3$ GeV \\
\hline
$\text{BR}(b\rightarrow s\gamma)$ & $(343\pm21\pm7) \times 10^{-6}$ & \cite{Amhis:2014hma} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $40\%$ \\
$\text{BR}(B_s\rightarrow\mu^+\mu^-)$ & $(2.8^{+0.7}_{-0.6})\times10^{-9}$ & \cite{CMS:2014xfa} & \texttt{susyflavor}\cite{Crivellin:2012jv} & $20\%$ \\
$\text{BR}(B_d\rightarrow\mu^+\mu^-)$ & $(3.9^{+1.6}_{-1.4})\times10^{-10}$ & \cite{CMS:2014xfa} & \texttt{susyflavor}\cite{Crivellin:2012jv} & $20\%$ \\
$\text{BR}(B\rightarrow\tau\nu)$ & $(114\pm22)\times10^{-6}$ & \cite{Amhis:2014hma} & \texttt{susyflavor}\cite{Crivellin:2012jv} & $50\%$ \\
\hline
$\text{BR}(B \rightarrow K^*\mu^+\mu^-)_{1\leq q^2\leq 6\ \text{GeV}^2}$  &  $0.34\pm0.03\pm0.04\pm0.02^{+0.00}_{-0.03}\times10^{-7}$ & \cite{Aaij:2013iag} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $105\%$ \\
$\text{BR}(B \rightarrow K^*\mu^+\mu^-)_{14.18\leq q^2\leq 16\ \text{GeV}^2}$ & $0.45\pm0.06\pm0.04\pm0.04^{+0.00}_{-0.05}\times10^{-7}$ & \cite{Aaij:2013iag} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $190\%$ \\
$q_0^2(\text{A}_\text{FB}(B \rightarrow K^*\mu^+\mu^-))$     &  $4.9\pm0.9 \text{GeV}^2$ & \cite{Aaij:2013iag} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $25\%$ \\
$F_L(B \rightarrow K^*\mu^+\mu^-)_{1\leq q^2\leq 6\ \text{GeV}^2}$ & $0.65^{+0.08+0.03}_{-0.07-0.03}$ & \cite{Aaij:2013iag} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $45\%$ \\
$F_L(B \rightarrow K^*\mu^+\mu^-)_{14.18\leq q^2\leq 16\ \text{GeV}^2}$ & $0.33^{+0.08+0.03}_{-0.07-0.03}$ & \cite{Aaij:2013iag} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $80\%$ \\
$-2P_2=A_T^\text{Re}(B \rightarrow K^*\mu^+\mu^-)_{1\leq q^2\leq 6\ \text{GeV}^2}$ & $-0.66^{+0.24+0.04}_{-0.22-0.01}$ & \cite{Aaij:2013iag} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $95\%$ \\
$-2P_2=A_T^\text{Re}(B \rightarrow K^*\mu^+\mu^-)_{14.18\leq q^2\leq 16\ \text{GeV}^2}$ & $1.00^{+0.00+0.00}_{-0.05-0.02}$ & \cite{Aaij:2013iag} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $45\%$ \\
$P_4'(B \rightarrow K^*\mu^+\mu^-)_{1\leq q^2\leq 6\ \text{GeV}^2}$ & $0.58^{+0.36}_{-0.32}\pm0.06$ & \cite{Aaij:2013qta} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $30\%$ \\ %*-2
$P_4'(B \rightarrow K^*\mu^+\mu^-)_{14.18\leq q^2\leq 16\ \text{GeV}^2}$ & $-0.18^{+0.70}_{-0.54}\pm0.08$ & \cite{Aaij:2013qta} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $35\%$ \\ %*-2
$P_5'(B \rightarrow K^*\mu^+\mu^-)_{1\leq q^2\leq 6\ \text{GeV}^2}$ & $0.21^{+0.20}_{-0.21}\pm0.03$ & \cite{Aaij:2013qta} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $45\%$ \\
$P_5'(B \rightarrow K^*\mu^+\mu^-)_{14.18\leq q^2\leq 16\ \text{GeV}^2}$ & $-0.79^{+0.20}_{-0.13}\pm0.18$ & \cite{Aaij:2013qta} & \texttt{superiso}\cite{Mahmoudi:2008tp} & $60\%$ \\
\hline
\end{tabular}
}
\end{center}
\caption{\small This table includes 45 observables that we fit.  All experimental errors are $1\sigma$ unless otherwise indicated.  Column 4 shows the software package that gives us the theoretical prediction.  $M_Z$ is fit precisely to impose electroweak symmetry breaking.  To account for the inconsistencies in the inclusive and exclusive measurements of $|V_{ub}|$ and $|V_{cb}|$, we perform the global $\chi^2$ analysis using the inclusive and exclusive measurements separately.  We also perform an additional analysis where the error bars of $|V_{ub}|$ and $|V_{cb}|$ cover both the inclusive and exclusive values.  In additional to the theoretical errors indicated in \texttt{superiso} manual, we added an additional 15\% error to each of the $B\to K^*\mu^+\mu^-$ observables because \texttt{superiso} does not take into account the phases of soft terms.}
\label{tab:obs}
\end{table}

==> SO(10) New/tables/prediction.tex <==
\begin{table}[!htbp]
  \begin{center}
    \begin{tabular}{| l | r | r | r | r |}
      \hline $m_{16}$ & 25 & 25 & 25 & 25 \\
      $\alpha$ & 0 & 1.5 & 0 & 1.5 \\
      \hline $\chi^2$/d.o.f & 2.158 & 2.275 & 2.220 & 2.505 \\
      \hline $m_{\tilde t_1}$ & 4.903 & 5.011 & 4.909 & 5.249 \\
      $m_{\tilde t_2}$ & 6.021 & 6.120 & 6.033 & 6.301 \\
      $m_{\tilde b_1}$ & 5.989 & 6.088 & 6.455 & 6.606 \\
      $m_{\tilde b_2}$ & 6.454 & 6.541 & 6.445 & 6.267 \\
      $m_{\tilde\tau_1}$ & 9.880 & 9.931 & 9.912 & 10.040 \\
      $m_{\tilde\tau_2}$ & 15.369 & 15.365 & 15.393 & 15.516 \\
      $M_{\tilde g}$ & 1.202 & 1.187 & 1.613 & 1.690 \\
      $m_{\tilde\chi_1^0}$ & 0.203 & 0.551 & 0.279 & 0.900 \\
      $m_{\tilde\chi_2^0}$ & 0.404 & 0.665 & 0.538 & 1.018 \\
      $m_{\tilde\chi_1^+}$ & 0.404 & 0.665 & 0.538 & 1.018 \\
      $m_{\tilde\chi_2^+}$ & 1.128 & 1.243 & 1.232 & 1.537 \\
      $M_A$ & 2.194 & 2.082 & 2.477 & 3.352 \\
      \hline $\sin\delta$ & -0.289 & -0.482 & -0.520 & -0.576 \\
      $BR(\mu\to e\gamma)\times10^{13}$ & 1.108 & 1.430 & 1.239 & 1.340 \\
      $\text{edm}_e\times10^{30}(\text{e cm})$ & -1.403 & -3.305 & -1.763 & -5.886 \\
      \hline
    \end{tabular}
    \caption{Predictions with $m_{16}=25\ \text{TeV}$ for $M_{\tilde g} \approx 1.2\ \text{TeV}$ and $1.6\ \text{TeV}$.  All masses in the table are in TeV units.  Our prediction for the branching ratio $\mu\to e\gamma$ is consistent with the current upper bound of $5.7 \times 10^{-13}$ \cite{Agashe:2014kda}.   In addition, our prediction of the electron electric dipole moment is consistent with the current upper bound of $10.5 \times10^{-28}\ \text{e cm}$ \cite{Agashe:2014kda}.}
    \label{tab:prediction}
  \end{center}
\end{table}

==> SO(10) New/tables/trend.tex <==
\begin{table}[!htbp]
  \begin{center}
    \begin{tabular}{| l | r | r | r | r | r |}
      \hline & \multicolumn{5}{c|}{Pull} \\
      \cline{2-6} $m_{16}$ & 10 & 15 & 20 & 25 & 30 \\
      \hline $M_W$ & 0.2110 & 0.1878 & 0.1851 & 0.2320 & 0.3981 \\
      \hline $M_h$ & 2.5474 & 1.1795 & 0.3454 & 0.1882 & 0.6582 \\
      \hline $BR(B\to\tau\nu)$ & 1.1978 & 1.3952 & 1.3557 & 1.3588 & 1.3771 \\
      \hline $F_L(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.2696 & 0.2488 & 0.2219 & 0.2101 & 0.2057 \\
      $P_4'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 1.7066 & 1.7066 & 1.7066 & 1.7066 & 1.7066 \\
      $P_5'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 2.4110 & 2.3432 & 2.2746 & 2.2451 & 2.2339 \\
      \hline $\chi^2$ & 14.1511 & 8.9744 & 7.2154 & 7.0206 & 7.5220 \\
      \hline
    \end{tabular}

    \vspace{0.5cm}
    {\footnotesize
    \begin{tabular}{| l | r | r | r | r | r | r |}
      \hline & \multicolumn{5}{c|}{Fit Value} & Exp. \\
      \cline{2-6} $m_{16}$ & 10 & 15 & 20 & 25 & 30 & Value \\
      \hline $M_W$ & 80.4699 & 80.4606 & 80.4595 & 80.4784 & 80.5454 & 80.3850 \\
      \hline $M_h$ & 117.9901 & 122.1303 & 124.6547 & 126.2697 & 127.6920 & 125.7000 \\
      \hline $BR(B\to\tau\nu)\times10^5$ & 6.6329 & 6.1340 & 6.2299 & 6.2223 & 6.1778 & 11.4000 \\
      \hline $F_L(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.7434 & 0.7353 & 0.7251 & 0.7207 & 0.7191 & 0.6500 \\
      $P_4'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & 0.8174 & 0.6711 & 0.5921 & 0.5717 & 0.5657 & 0.5800 \\
      $P_4'(B\to K^*\mu^+\mu^-)_{14.18\leq q^2\leq16\ \text{GeV}^2}$ & 1.2190 & 1.2190 & 1.2190 & 1.2190 & 1.2190 & -0.1800 \\
      $P_5'(B\to K^*\mu^+\mu^-)_{1\leq q^2\leq6\ \text{GeV}^2}$ & -0.7301 & -0.5529 & -0.4625 & -0.4335 & -0.4235 & 0.2100 \\
      \hline
    \end{tabular}
    }
    \caption{This table shows the set of observables with $\alpha=0$ and $M_{\tilde g}\approx1.2\ \text{TeV}$.  As argued by Altmannshofer et.~al.  $B\to K^*\mu^+\mu^-$ favors large $m_{\tilde t}$ \cite{Altmannshofer:2013foa}, which is in agreement with our analysis.  On the other hand, as explained in the text, fitting to $M_W$ and $M_h$ disfavors large $m_{\tilde t}$.  These effects collectively contribute to having a minimum $\chi^2$ around $m_{16}=25\ \text{TeV}$. The $\chi^2$ value is plotted as a function of $m_{16}$ in Figure \ref{fig:trend}.  In addition to the observables contributing directly to a minimum of $\chi^2$ at $m_{16}=25\ \text{TeV}$, also included in this table is the calculated value of $P_4'$ at high $q^2$ bin.  This is to illustrate that the value of $P_4'$ does not depend on the $m_{16}$, which again agrees with previous analysis~\cite{Altmannshofer:2013foa, Descotes-Genon:2013wba}.}
    \label{tab:trend}
  \end{center}
\end{table} 
